The chirally rotated Schr\"odinger functional with Wilson fermions and automatic O(a) improvement

A modified formulation of the Schr\"odinger functional (SF) is proposed. In the continuum it is related to the standard SF by a non-singlet chiral field rotation and therefore referred to as the chirally rotated SF ($\chi$SF). On the lattice with Wilson fermions the relation is not exact, suggesting some interesting tests of universality. The main advantage of the $\chi$SF consists in its compatibility with the mechanism of automatic O($a$) improvement. In this paper the basic set-up is introduced and discussed. Chirally rotated SF boundary conditions are implemented on the lattice using an orbifold construction. The lattice symmetries imply a list of counterterms, which determine how the action and the basic fermionic two-point functions are renormalised and O($a$) improved. As with the standard SF, a logarithmically divergent boundary counterterm leads to a multiplicative renormalisation of the fermionic boundary fields. In addition, a finite dimension 3 boundary counterterm must be tuned in order to preserve the chirally rotated boundary conditions in the interacting theory. Once this is achieved, O($a$) effects originating from the bulk action or from insertions of composite operators in the bulk can be avoided by the mechanism of automatic O($a$) improvement. The remaining O($a$) effects arise from the boundaries and can be cancelled by tuning a couple of O($a$) boundary counterterms. The general results are illustrated in the free theory where the Sheikholeslami-Wohlert term is shown to affect correlation functions only at O($a^2$), irrespective of its coefficient.

==> section3_tmp.tex <==
\section{Continuum considerations}

The boundary conditions involving the projectors $\tilde{Q}_\pm$   
can be thought of as a chirally rotated version of the standard SF boundary conditions.
As the non-singlet chiral rotation is part of the continuum symmetries of 
massless QCD, the alternative formulation of the SF to be introduced here 
will in fact be closely related to the standard SF. It is useful to have a closer look
at this relationship before passing to the lattice formulation.

\subsection{Chirally rotated SF boundary conditions}

Let $\psi'$ and $\psibar'$ be isospin doublets  
of quark and anti-quark fields satisfying the homogeneous 
SF boundary conditions, Eq.(\ref{eq:SFbcs}).
Performing a non-singlet chiral field rotation,
\begin{equation}
    \psi'= R(\alpha)\psi,\qquad \psibar'=\psibar R(\alpha), \qquad 
     R(\alpha)=\exp(i\alpha \gamma_5\tau^3/2),
 \label{eq:chiral_rot}
\end{equation}
the rotated fields satisfy the chirally rotated boundary conditions,
\begin{xalignat}{2}
     P_+(\alpha)\psi(x)\vert_{x_0=0} &=0,    
    &P_-(\alpha)\psi(x)\vert_{x_0=T} &=0,\nonumber\\
   \psibar(x)\gamma_0P_-(\alpha)\vert_{x_0=0} &= 0,   
    &\psibar(x)\gamma_0P_+(\alpha)\vert_{x_0=T} &= 0, 
\label{eq:rotbc}
\end{xalignat}
with the projectors
\begin{equation}
  P_\pm(\alpha)=\frac12\left[1\pm\gamma_0\exp(i\alpha\gamma_5\tau^3)\right].
\end{equation}
For $\alpha=0$ the standard projectors $P_\pm=P_\pm(0)$ are recovered,
while for $\alpha=\pi/2$ one finds,
\begin{equation}
   P_\pm(\pi/2)\equiv \tilde{Q}_\pm=\frac12(1\pm i\gamma_0\gamma_5\tau^3).
\end{equation}
Since $\gamma_0 \tilde{Q}_\pm=\tilde{Q}_\mp\gamma_0$, the boundary
conditions (\ref{eq:rotbc}) in this special case read
\begin{xalignat}{2}
     \tilde{Q}_+\psi(x)\vert_{x_0=0} &=0,    
    &\tilde{Q}_-\psi(x)\vert_{x_0=T} &=0,\nonumber\\
   \psibar(x)\tilde{Q}_+\vert_{x_0=0} &= 0,   
    &\psibar(x)\tilde{Q}_-\vert_{x_0=T} &= 0.
\label{eq:bc_rotate}
\end{xalignat}
We thus see that boundary conditions involving the projectors $\tilde{Q}_\pm$ 
appear naturally when chirally rotating quark and anti-quark fields 
which satisfy the standard SF boundary conditions.

\subsection{Properties of the continuum Dirac operator}

In the continuum the rotation angle $\alpha$ parameterizes a 
family of linear spaces of functions
which satisfy homogeneous Dirichlet boundary conditions
in Euclidean time. In the spatial direction we assume $L$-periodicity and we
allow for a constant U(1) gauge background field $i\theta_\mu/L$.
Formally this field may be included in the Dirac operator 
by promoting the SU($N$) colour gauge field to a U($N$) gauge field as follows:
\be
   A_\mu(x)= \sum_{a=0}^{N^2-1} A_\mu^a(x) T^a,\qquad  A_\mu^{0}(x) T^0 =  i\frac{\theta_\mu}{L} \Id.
\ee
Following~\cite{Sint:1995ch,Luscher:1996sc}, we usually set $\theta_1=\theta_2=\theta_3=\theta$ and $\theta_0=0$.  
With respect to the natural inner product,
\begin{equation}
    (\varphi,\chi) = \int_0^T\rmd x_0\int\rmd^3\bfx\, \varphi(x)^\dagger \chi(x),
\end{equation}
the Dirac operator for a quark doublet and generic angle $\alpha$ is $\gamma_5$-hermitian up to a flavour 
exchange, i.e.
\begin{equation}
   \left(\gamma_5\tau^1\left[\Dslash+m+i\muq\gamma_5\tau^3\right]\right)^\dagger = 
         \gamma_5\tau^1\left[\Dslash+m+i\muq\gamma_5\tau^3\right].
\end{equation}
For later reference both a standard and a twisted mass term have been included.
Hence, a well-defined eigenvalue problem is obtained for any value\footnote{As an aside 
note that for $\alpha=\pi/2$ the massless operator $i\Dslash$ is hermitian for a single fermion
with boundary conditions corresponding to either the up or the down flavour in Eq.~(\ref{eq:bc_rotate}).} 
of $\alpha$.
Denoting the  eigenfunctions in the standard SF bei $v_n$, the eigenvalue equation reads
\begin{equation}
   \gamma_5\tau^1\left[\Dslash+m+i\muq\gamma_5\tau^3\right] v_n = \lambda_n v_n.
\end{equation}
Performing the chiral rotation as in Eq.(\ref{eq:chiral_rot}), 
\begin{equation}
    v_n = R(\alpha)w_n
\end{equation}
and using 
\begin{eqnarray}
  R(\alpha)\left[\Dslash+m+i\muq\gamma_5\tau^3\right] R(\alpha) &=& 
   \Dslash+\tilde{m}+i\tilde{\muq}\gamma_5\tau^3,
\end{eqnarray}
one finds,
\begin{equation}
 \gamma_5\tau^1 \left[\Dslash+\tilde{m}+i\tilde{\muq}\gamma_5\tau^3\right] w_n = \lambda_n w_n.
\end{equation}
Hence, the eigenfunctions are related by a chiral rotation, and the eigenvalues are exactly the same
as in the standard SF, provided the mass parameters either vanish or are transformed covariantly,
according to
\begin{equation}
 \tilde{m} =
 m\cos\alpha -\mu_q\sin\alpha,
 \qquad
 \tilde{\mu_q} =
 m\sin\alpha +\mu_q\cos\alpha.
\label{eq:cov_mass}
\end{equation}
Moreover, the absence of zero modes in the massless theory can be established following 
L\"uscher~\cite{Luscher:2006df}, and some details have been deferred to Appendix~A.
Given the absence of zero modes, the free continuum quark propagator can then be 
calculated using standard techniques. Some results are collected in Appendix~B.


\subsection{Relating correlation functions at different values of $\alpha$}

The chiral rotation (\ref{eq:chiral_rot}) is not anomalous, so that
one may perform a corresponding change of variables in the functional integral. 
One obtains relations between correlation functions
defined with the standard and the chirally rotated SF boundary conditions.
This is similar to and generalises the relations between correlation functions in 
twisted mass and standard QCD~\cite{Frezzotti:2000nk,Sint:2007ug}. 
In particular, one expects that these formal continuum relations will hold up to cutoff effects, 
for appropriately renormalised correlation functions on the lattice.

It is instructive to include both a standard
and a twisted mass term in the fermionic action at $\alpha=0$, 
\begin{equation}
 S_f[m,\muq] = \int_0^T{\rm d}x_0 \int_0^L{\rm d}^3{\bf x}\,\,
  \psibar'(x)(\Dslash+m+i\muq\gamma_5\tau^3)\psi'(x),
\end{equation}
even though the focus will later be on massless QCD.
Performing the change of variables, Eq.~(\ref{eq:chiral_rot}),
one obtains the generic identities,
\begin{eqnarray}
 \left\langle O[\psi,\psibar]\right\rangle_{(m,\muq,P_{\pm})}=
 \left\langle O[R(\alpha)\psi,\psibar R(\alpha)]\right\rangle_{
        (\tilde{m},\tilde{\mu}_q,P_{\pm}(\alpha))},
\label{eq:equivSF}
\end{eqnarray}
where the integration variables are assumed to be $\psi$ and $\psibar$ 
on both sides of the equation.  In addition to the boundary conditions for $\psi$ at $x_0=0,T$,
the subscript to the correlation functions indicates the mass parameters in the action and
the mass parameters are related as in Eq.~(\ref{eq:cov_mass}).

The relation~(\ref{eq:equivSF}) establishes a mapping of correlation functions
defined at different values of $\alpha$.  An equivalent form of this mapping is given by
\begin{equation}
 \left\langle O[\psi,\psibar]\right\rangle_{(\tilde{m},\tilde{\mu}_{\rm q},\tilde{Q}_{\pm})}=
 \left\langle O[R(-\alpha)\psi,\psibar R(-\alpha)]
      \right\rangle_{(m,\muq,P_{\pm}(\frac{\pi}{2}-\alpha))}.
\label{eq:equivSFp}
\end{equation}
Setting the twisted mass term to zero in the
chirally rotated  SF, and choosing $\alpha=\pi/2$, this simplifies to
\begin{equation}
 \langle O[\psi,\psibar]\rangle_{(m,0,\tilde{Q}_{\pm})}=
 \langle O[R(-\pi/2)\psi,\psibar R(-\pi/2)]\rangle_{(0,-m,P_\pm)},
\end{equation}
which shows that the standard mass parameter in the chirally rotated SF
is equivalent to a (negative) twisted mass parameter in the standard SF.

The simplest fermionic correlation function is the quark propagator. 
Using the explicit expressions of Appendix~B,
one may easily verify the identity (\ref{eq:chiral_rot}) in the free theory, viz.
\begin{equation}
   \left\langle \psi(x)\psibar(y) \right\rangle_{(m,\muq,P_\pm)}^{(g=0)} =
   R(\alpha) \left\langle \psi(x)\psibar(y) \right\rangle^{(g=0)}_{(\tilde{m},\tilde{\mu}_{\rm q},P_\pm(\alpha))} R(\alpha).
\end{equation}
Gauge invariant correlation functions corresponding 
to the ones defined in the standard SF~\cite{Luscher:1996sc,Luscher:1996vw} 
can be defined as well. For this we need the fermionic boundary fields, 
$\zeta,\zetaprime$ and $\zetabar,\zetabarprime$, which are naturally included in the mapping~(\ref{eq:equivSF})  
by identifying them with the non-Dirichlet components near the time boundaries.
More precisely we set
\begin{xalignat}{2}
     \zeta(\bfx) &=  P_-(\alpha)\psi(0,\bfx),    
    &\zetaprime(\bfx) &= P_+(\alpha)\psi(T,\bfx),\nonumber\\
     \zetabar(\bfx) &= \psibar(0,\bfx)P_+(-\alpha), 
    &\zetabarprime(\bfx)&= \psibar(T,\bfx) P_-(-\alpha),  
\label{eq:zeta_alpha}
\end{xalignat}
thus leaving the $\alpha$-dependence implicit.
This should not lead to any confusion, as these fields mostly appear 
as insertions into correlation functions with subscripts indicating the projectors 
used for the boundary conditions.

\subsection{Symmetries and conventions}

The standard SF boundary conditions break all chiral symmetries, as 
is best illustrated by the Ward identities~\cite{Luscher:2006df}.
With the global axial and vector non-singlet variations,
\begin{xalignat}{2}
     \delta_{\rm A}^a\psi &= \gamma_5\frac{\tau^a}{2}\psi,    
    &\delta_{\rm V}^a\psi &= \frac{\tau^a}{2}\psi, \nonumber\\
     \delta_{\rm A}^a\psibar &= \psibar \gamma_5\frac{\tau^a}{2}, 
    &\delta_{\rm V}^a\psibar &= -\psibar \frac{\tau^a}{2}, 
\end{xalignat}
the Ward identities take the form,
\begin{equation}
    \langle \delta_{\rm X}^a O\rangle_{(P_\pm)} =  \langle \delta_{\rm X}^a S\rangle,\qquad {\rm X}={\rm A,V},
\end{equation}
and the variations of the action are given by
\begin{equation}
   \delta_{\rm A} S = -\int\rmd^4x \partial_\mu A_\mu^a(x),\qquad \delta_{\rm V} S = -\int\rmd^4x \partial_\mu V_\mu^a(x),
\end{equation}
with the Noether currents
\begin{equation}
  A_\mu^a(x) = \psibar(x)\gamma_\mu\gamma_5\frac{\tau^a}{2}
\end{equation}




\begin{eqnarray}
 \langle \delta_{\rm A}^a O\rangle_{(P_\pm)} &=& 
    \half\int \rmd^3z\left\langle \left[\zetabar(\bfz)\gamma_5\tau^a\zeta(\bfz) +
          \zetabarprime(\bfz)\gamma_5\tau^a\zetaprime(\bfz)\right] O\right\rangle_{(P_\pm)},\\
    \langle  \delta_{\rm V}^a O\rangle_{(P_\pm)} &=& 0.
\end{eqnarray}
Here, $O$ denotes an arbitrary polynomial in the fields, and the subscript to the expectation values
indicates the boundary conditions for $\psi$ at $x_0=0,T$.
The Ward identities show that the standard SU(2) vector symmetry is conserved, 
while the breaking of chiral symmetry is analogous to the breaking by a standard
mass term, except that the breaking terms are localized at the time boundaries, with coefficients
of O($1$). In particular, this means that any Ward identity obtained from local variations 
inside the volume will reflect the complete bulk symmetries of massless QCD.

It is straightforward to derive the corresponding equations 
for chirally rotated SF boundary conditions,
\begin{eqnarray}
 \langle \delta_{\rm A}^a O\rangle_{(P_\pm(\alpha))}\! &=& \!
   \half\! \int \rmd^3z\left\langle \left[\zetabar(\bfz)\gamma_0\gamma_5\tau^a\zeta(\bfz) -
          \zetabarprime(\bfz)\gamma_0\gamma_5\tau^a\zetaprime(\bfz)\right] O\right\rangle_{(P_\pm(\alpha))},
\label{eq:AWI}\\
  \langle \delta_{\rm V}^a O\rangle_{(P_\pm(\alpha))} \!&=& \!
   \half\! \int \rmd^3z\left\langle \left[\zetabar(\bfz)\gamma_0\tau^a\zeta(\bfz) -
          \zetabarprime(\bfz)\gamma_0\tau^a\zetaprime(\bfz)\right] O\right\rangle_{(P_\pm(\alpha))}.
\label{eq:VWI}
\end{eqnarray}
Using the projector structure implicit in the fermionic boundary fields, Eq.~(\ref{eq:zeta_alpha}), 
the r.h.s.~of the vector Ward identity (\ref{eq:VWI}) with index $a=3$ is seen to vanish. 
Moreover, there are two further linear combinations of Eqs.~(\ref{eq:AWI},\ref{eq:VWI}) for which 
the r.h.s.~vanishes, so that three generators correspond to conserved symmetries.
This is not surprising, as the  chiral rotation merely transforms the vector symmetry 
of the standard SF to an unusual form, a situation which is familiar 
from twisted mass QCD~\cite{Frezzotti:2000nk,Sint:2007ug}.

To illustrate this further, consider the case of most interest, $\alpha=\pi/2$, where the 
Ward identities take the form
\begin{eqnarray}
 \langle \delta_{\rm A}^{a} O\rangle_{(\tilde{Q}_\pm)} &=& \tfrac{i}{2}\delta^{3a}
           \int \rmd^3z\left\langle \left[\zetabar(\bfz)\zeta(\bfz) +
          \zetabarprime(\bfz)\zetaprime(\bfz)\right] O\right\rangle_{(\tilde{Q}_\pm)},
\label{eq:ward1}\\
  \langle \delta_{\rm V}^{a} O\rangle_{(\tilde{Q}_\pm)} &=& \tfrac{i}{2}\varepsilon^{3ab}
    \int \rmd^3z\left\langle \left[\zetabar(\bfz)\gamma_5\tau^{b}\zeta(\bfz) -
          \zetabarprime(\bfz)\gamma_5\tau^b\zetaprime(\bfz)\right] O\right\rangle_{(\tilde{Q}_\pm)}.
\label{eq:ward2}
\end{eqnarray}
Apparently a mixture of vector and axial symmetries are broken by 
boundary terms. However, in massless QCD this is really a convention dependent statement.
A preferred or ``physical" basis is only available in the presence of a mass term: 
those symmetry transformations leaving the mass term invariant are identified as 
vector symmetries whereas the remaining chiral flavour transformations are classified as axial symmetries. 
In massless QCD with SF type boundary conditions we will choose a similar convention, and define
the ``physical" basis as the one with standard SF boundary conditions. This implies that 
the broken symmetries are in all cases the axial symmetries, whereas the vector or isospin symmetries
are conserved. The situation is then completely analogous to twisted mass QCD, in particular, the ``dictionary"
translating composite fields between both bases can be taken over from twisted mass QCD.

